Higher homological algebra for one-point extensions of bipartite hereditary algebras and spectral graph theory

In this article we study higher homological properties of $n$-levelled algebras and connect them to properties of the underlying graphs. Notably, to each $2$-representation-finite quadratic monomial algebra $\Lambda$ we associate a bipartite graph $\overline{B_{\Lambda}}$ and we classify all such algebras $\Lambda$ for which $\overline{B_{\Lambda}}$ is regular or edge-transitive. We also show that if $\overline{B_{\Lambda}}$ is semi-regular, then it is a reflexive graph.

==> Sections/C-correspondence_between_solutions.tex <==

\begin{proof}
Using Proposition \ref{prop:determinant of block matrix}(a) we compute
\begin{align*}
    \CP_{A}(\lambda) &= \det 
\begin{bmatrix}
\lambda I_r & -R \\
-R^T & \lambda I_s
\end{bmatrix} \\
&= \det(\lambda I_r)\det(\lambda I_s-(-R^T)(\lambda I_r)^{-1}(-R)) \\
&= \lambda^{r}\det(\lambda I_s - \lambda^{-1}R^T R).
\end{align*}


Making the substitution $\lambda = \sqrt{z} + \frac{1}{\sqrt{z}}$, we obtain
\begin{equation}\label{eq:q(sqrt(t)+1/sqrt(t)}
    \CP_{A}\left(\sqrt{z}+\frac{1}{\sqrt{z}}\right)= (z+1)^r z^{-\frac{r}{2}}\det((z+1)z^{-\frac{1}{2}}I_s - (z+1)^{-1}z^{\frac{1}{2}}R^TR).
\end{equation}
On the other hand, using Proposition \ref{prop:main properties of setup}(a) we have
\begin{align*}
    \CP_{\K Q}(z) =\det(zC_{\K Q}+C_{\K Q}^T) =\det\begin{bmatrix}
    (z+1)I_r & zR \\
    R^T & (z+1)I_s
    \end{bmatrix}.
\end{align*}
Using Proposition \ref{prop:determinant of block matrix}(a) we obtain
\begin{align*}
    \CP_{\K Q}(z) 
    & = \det((z+1)I_r) \det((z+1)I_s - R^T((z+1)I_r)^{-1} zR)\\
    & = (z+1)^r \det((z+1)I_s - (z+1)^{-1}zR^T R)\\
    & = (z+1)^r \det(z^{\frac{1}{2}}((z+1)z^{-\frac{1}{2}}I_s-(z+1)^{-1}z^{\frac{1}{2}}R^T R))\\
    & = (z+1)^{r} z^{\frac{s}{2}}\det((z+1)z^{-\frac{1}{2}}I_s - (z+1)^{-1}z^{\frac{1}{2}}R^T R)\\
    & \overset{(\ref{eq:q(sqrt(t)+1/sqrt(t)})}{=} (z+1)^{r} z^{\frac{s}{2}}\frac{\CP_{A}\left(\sqrt{z}+\frac{1}{\sqrt{z}}\right)}{(z+1)^r z^{-\frac{r}{2}}}  \\
    &=z^{\frac{r+s}{2}}\CP_{A}\left(\sqrt{z}+\frac{1}{\sqrt{z}}\right).
\end{align*}
Hence, we see that every pair of solutions $\{z, z^{-1}\}$ of $\CP_{\K Q}$ corresponds to a pair of solutions $\{\lambda, -\lambda\}$ of $\CP_A$. 
Indeed, as $A$ is bipartite, we have $\CP_A(\lambda) = 0$ if and only if $\CP_A(-\lambda) = 0$. 
Moreover, note that 
\[
z + \frac{1}{\sqrt{z}} = z^{1/2}+ \frac{1}{z^{1/2}} = \frac{1}{z^{-1/2}} z^{-1/2} = \frac{1}{\sqrt{z}} + z.
\]
On the other hand, solving 
\[
\lambda = \sqrt{z}+\frac{1}{\sqrt{z}}
\]
for $z$, we have 
\[
z = \frac{\left(\lambda^2-2\right)\pm \lambda\sqrt{\lambda^2-4}}{2},
\]
and it is straightforward to check that the solutions this yields are inverse to each other, even in case they are not distinct, i.e.\ when $\lambda \in \{0, \pm 2\}$.
\end{proof}
